A variational study of two-nucleon systems with lattice QCD

The low-energy spectrum and scattering of two-nucleon systems are studied with lattice quantum chromodynamics using a variational approach. A wide range of interpolating operators are used: dibaryon operators built from products of plane-wave nucleons, hexaquark operators built from six localized quarks, and quasi-local operators inspired by two-nucleon bound-state wavefunctions in low-energy effective theories. Sparsening techniques are used to compute the timeslice-to-all quark propagators required to form correlation-function matrices using products of these operators. Projection of these matrices onto irreducible representations of the cubic group, including spin-orbit coupling, is detailed. Variational methods are applied to constrain the low-energy spectra of two-nucleon systems in a single finite volume with quark masses corresponding to a pion mass of 806 MeV. Results for S- and D-wave phase shifts in the isospin singlet and triplet channels are obtained under the assumption that partial-wave mixing is negligible. Tests of interpolating-operator dependence are used to investigate the reliability of the energy spectra obtained and highlight both the strengths and weaknesses of variational methods. These studies and comparisons to previous studies using the same gauge-field ensemble demonstrate that interpolating-operator dependence can lead to significant effects on the two-nucleon energy spectra obtained using both variational and non-variational methods, including missing energy levels and other discrepancies. While this study is inconclusive regarding the presence of two-nucleon bound states at this quark mass, it provides robust upper bounds on two-nucleon energy levels that can be improved in future calculations using additional interpolating operators and is therefore a step toward reliable nuclear spectroscopy from the underlying Standard Model of particle physics.

==> GEVPspectrumI0T1_swave.tex <==
\begin{tabular}{|c|c|c|c|c|} \hline
$n$ & $a \Delta E_{\mathsf{n}}^{(2,0,T1,\mathbb{S}_0)}$ & $\Delta E_{\mathsf{n}}^{(2,0,T1,\mathbb{S}_0)}\text{ [MeV]}$ & $k_{\matsf{n}}^{(2,0,T_1^+,\mathbb{S}_0)^2}/m_\pi^2$ & $k_n^{(2,0,T_1^+,\mathbb{S}_0)}/m_\pi \cot\delta_{\ell=0}^{(2,0)}$ \\\hline
0 & $-0.0027(4.0000)$ & $-3.7(0.6)$ & $-0.0093(15)$ & $0.02\left(_{-5}^{2}\right)$ \\\hline
1 & $0.0216(9.0000)$ & $29.3(1.3)$ & $0.0739(31)$ & $0.18\left(_{-22}^{14}\right)$ \\\hline
2 & $0.0523(8.0000)$ & $71.0(1.3)$ & $0.1026(15)$ & $0.34\left(_{-40}^{29}\right)$ \\\hline
3 & $0.0861(7.0000)$ & $116.9(1.6)$ & $0.1803(28)$ & $0.23\left(_{-27}^{17}\right)$ \\\hline
4 & $0.1149(10.0000)$ & $156.1(2.2)$ & $0.2021(22)$ & $0.22\left(_{-27}^{16}\right)$ \\\hline
5 & $0.1410(14.0000)$ & $191.5(2.8)$ & $0.2029(23)$ & $0.66\left(_{-78}^{54}\right)$ \\\hline
6 & $0.1706(15.0000)$ & $231.7(3.2)$ & $0.2988(23)$ & $-0.06\left(_{-9}^{23}\right)$ \\\hline
7 & $0.1723(17.0000)$ & $234.0(3.4)$ & $0.3044(26)$ & $0.14\left(_{-31}^{7}\right)$ \\\hline
\end{tabular}

==> GEVPspectrumI1A1_swave.tex <==
\begin{tabular}{|c|c|c|c|c|} \hline
$n$ & $a \Delta E_{\mathsf{n}}^{(2,1,A1,\mathbb{S}_0)}$ & $\Delta E_{\mathsf{n}}^{(2,1,A1,\mathbb{S}_0)}\text{ [MeV]}$ & $k_{\matsf{n}}^{(2,1,A_1^+,\mathbb{S}_0)^2}/m_\pi^2$ & $k_n^{(2,1,A_1^+,\mathbb{S}_0)}/m_\pi \cot\delta_{\ell=0}^{(2,1)}$ \\\hline
0 & $-0.0026(5.0000)$ & $-3.5(0.7)$ & $-0.0087(17)$ & $0.04\left(_{-8}^{2}\right)$ \\\hline
1 & $0.0225(11.0000)$ & $30.5(1.5)$ & $0.0770(36)$ & $0.22\left(_{-26}^{17}\right)$ \\\hline
2 & $0.0533(9.0000)$ & $72.4(1.5)$ & $0.1839(32)$ & $0.41\left(_{-50}^{35}\right)$ \\\hline
3 & $0.0858(11.0000)$ & $116.6(1.9)$ & $0.2980(38)$ & $0.21\left(_{-30}^{10}\right)$ \\\hline
4 & $0.1158(12.0000)$ & $157.2(2.4)$ & $0.4044(42)$ & $0.27\left(_{-34}^{19}\right)$ \\\hline
5 & $0.1433(16.0000)$ & $194.6(3.0)$ & $0.5034(57)$ & $0.88\left(_{-105}^{67}\right)$ \\\hline
6 & $0.1713(17.0000)$ & $232.7(3.5)$ & $0.6053(62)$ & $0.02\left(_{-24}^{13}\right)$ \\\hline
\end{tabular}
